Human-In-The-Loop Learning of Qualitative Preference Models

In this work, we present a novel human-in-the-loop framework to help the human user understand the decision making process that involves choosing preferred options. We focus on qualitative preference models over alternatives from combinatorial domains. This framework is interactive: the user provides her behavioral data to the framework, and the framework explains the learned model to the user. It is iterative: the framework collects feedback on the learned model from the user and tries to improve it accordingly till the user terminates the iteration. In order to communicate the learned preference model to the user, we develop visualization of intuitive and explainable graphic models, such as lexicographic preference trees and forests, and conditional preference networks. To this end, we discuss key aspects of our framework for lexicographic preference models.

==> Makefile <==
PREFIX  = paper
TEXFILE = $(PREFIX).tex
PDFFILE = $(PREFIX).pdf
TMPFILE = .makedolatex.log

OPTIONS = -file-line-error -halt-on-error -interaction nonstopmode
#OPTIONS = -interaction nonstopmode

BLACK="\033[30m"
RED="\033[31m"
GREEN="\033[32m"
YELLOW="\033[33m"
BLUE="\033[34m"
PINK="\033[35m"
CYAN="\033[36m"
WHITE="\033[37m"
NORMAL="\033[0;39m"

ALLTEXFILES := $(shell ls *.tex)
BIBFILES := $(shell ls *.bib)
FIGFILES := $(shell ls figs/* | sed 's/ /\\ /g')


all:	$(PREFIX).pdf clean


$(PREFIX).pdf: $(PREFIX).tex $(ALLTEXFILES) $(BIBFILES) $(FIGFILES)
	@$(MAKE) dopdflatex;
	@$(MAKE) dobibtex;
	@$(MAKE) dopdflatex;
	@$(MAKE) dopdflatex;
	@echo;

.PHONY: dobibtex
dobibtex:
	@if ( grep bibdata\{ *.aux > /dev/null ); then \
		if ( grep citation\{ *.aux > /dev/null ); then \
			if ( bibtex $(PREFIX) > $(TMPFILE) ); then \
			 	printf $(GREEN); echo "(bibtex) OK"; \
			else \
				printf $(RED); echo "(bibtex) ERROR"; \
				cat $(TMPFILE); \
			fi; \
		fi; \
	fi;
	@printf $(NORMAL)

.PHONY: dopdflatex
dopdflatex:
	@if ( pdflatex --shell-escape $(OPTIONS) $(TEXFILE) > $(TMPFILE) ); then \
    printf $(YELLOW); \
	  grep Warning $(TMPFILE); \
		printf $(GREEN); echo "(pdflatex) OK"; \
  else \
	 	printf $(RED); \
		grep -A 6 "Error" $(TMPFILE); \
    echo "(...) last 20 lines of pdflatex output:";  \
	  tail -n 20 $(TMPFILE); \
    echo "(pdflatex) ERROR"; \
    echo; \
	fi;
	@printf $(NORMAL)

.PHONY: clean
clean:
	@if [ -f $(PREFIX).aux ]; then\
		rm $(PREFIX).aux;\
	fi
	@if [ -f $(PREFIX).log ]; then\
		rm $(PREFIX).log;\
	fi
	@if [ -f $(PREFIX).blg ]; then\
		rm $(PREFIX).blg;\
	fi
	@if [ -f $(PREFIX).bbl ]; then\
		rm $(PREFIX).bbl;\
	fi
	@if [ -f $(PREFIX).out ]; then\
		rm $(PREFIX).out;\
	fi
	@if [ -f $(PREFIX).tex.bak ]; then\
		rm $(PREFIX).tex.bak;\
	fi

.PHONY: spell
spell:
	aspell --lang=en --mode=tex check $(PREFIX).tex


==> results.tex <==
Show a couple of user case examples where the system interacts and iterates
to learn a preference tree model.
In this learning process, the user clearly see the improvement of the learned
model from iteration to iteration as the system adjusts each iteration according
to the user's feedback.

